Unsupervised Pose Flow Learning for Pose Guided Synthesis

Pose guided synthesis aims to generate a new image in an arbitrary target pose while preserving the appearance details from the source image. Existing approaches rely on either hard-coded spatial transformations or 3D body modeling. They often overlook complex non-rigid pose deformation or unmatched occluded regions, thus fail to effectively preserve appearance information. In this paper, we propose an unsupervised pose flow learning scheme that learns to transfer the appearance details from the source image. Based on such learned pose flow, we proposed GarmentNet and SynthesisNet, both of which use multi-scale feature-domain alignment for coarse-to-fine synthesis. Experiments on the DeepFashion, MVC dataset and additional real-world datasets demonstrate that our approach compares favorably with the state-of-the-art methods and generalizes to unseen poses and clothing styles.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> section/appendices.tex <==
\appendices
\section{Proof of the First Zonklar Equation}
Appendix one text goes here.

% you can choose not to have a title for an appendix
% if you want by leaving the argument blank
\section{}
Appendix two text goes here.

==> section/model.tex <==
\section{Approach}
\label{sec:approach}
We aim to generate an image that preserves the appearance of a source image $I_s$ and the pose of a target image $I_t$. We represent the poses of source and target images as $P_s$ and $P_t$, which are generated from $I_s$ and $I_t$, respectively,  by concatenating one-hot pose parsing and the corresponding mesh coordinate map of the results from Densepose~\cite{densepose}. In addition, the one-hot parsing of the source garment $C_s$ is extracted from $I_s$ using the method of~\cite{LIP}.

% Please refer to supplementary materials for more details.

As illustrated in Figure \ref{fig:pipeline}, a two-stage approach is proposed to transfer the appearance details from the source pose to the target pose for pose guided synthesis.
%to train the texture-preserving flow estimator for image synthesis. 
In Stage-\RNum{1}, a flow estimator is trained to capture pose deformations using the proposed unsupervised appearance preserving objective function. In Stage-\RNum{2}, the GarmentNet and SynthesisNet are designed to sequentially generate target garment parsing and final output in a coarse-to-fine manner. The GarmentNet and SynthesisNet share a unified network structure, which relies on the trained flow estimator for multi-scale feature domain alignment (as elaborated in Section \ref{subsection:method-stage2}). In addition, a multiplicative attention fusion module is  proposed to handle feature misalignment.

In Section \ref{subsection:method-stage1}, we describe the flow estimator and the unsupervised objective for training the appearance preserving flow. In Section \ref{subsection:method-stage2}, the GarmentNet and SynthesisNet as well as the  multiplicative attention fusion module are elaborated.

%Figure \ref{fig:model} summarizes the pipeline of our proposed. To ..., we first learning the texture preserving optical flow. Based on the learned flow, we present an two-stage network for pose-guided synthesis. The first stage aims to generate the cloth condition, while the second stage aims to perform final synthesis.

\begin{figure}[t]
	\centering
	\includegraphics[width=1.0\linewidth]{figures/flownetwork.pdf}
	\caption{The network structure of GarmentNet. Given the multi-scale flow fields from Stage-\RNum{1}, the garment encoding from the source image is spatially aligned to the target image using inversed warping. The target garment segmentation is then generated using the Unet decoder. The green, blue, yellow blocks indicate the source encoder, target encoder and Unet decoder, respectively.}
	\label{fig:flow_model}
\end{figure}


\subsection{Stage-\RNum{1}: Unsupervised Appearance Preserving Flow}
\label{subsection:method-stage1}
Instead of affine~\cite{deform_gan} or TPS transformation~\cite{CP-VTON,softgated}, we choose to learn an optical flow estimator to capture the pose deformation for appearance preserving transformation. As shown in Figure~\ref{fig:flow_model}, our flow estimator takes the source image, pose and target pose as inputs, and aims to generate a flow-field that describes the pose deformation.

More concretely, let ${Flow}$ denote a flow estimator that takes the source image $I_s$, source pose $P_s$, and target pose $P_t$ as inputs, and generates target-to-source flow-fields $V^{(i)}$ at multiple scales $i=[0,\dotsi ,5]$:
\begin{equation}
	\{V^{(0)}, V^{(1)}, \dotsi , V^{(4)}, V^{(5)}\} = {Flow}([I_s;P_s],P_t),
\label{equ:flow}
\end{equation} 
where $[\cdot;\cdot]$ denotes concatenation. We employ FlowNetS~\cite{flownet} as the baseline structure of the flow estimator. However, we only utilize the pose rather than the image from target domain since the target image can be quite different in appearance. FlowNetS is also adapted to improve the flow-field definition and to reduce memory usage. Please refer to supplementary material for more details.

Unsupervised flow training on natural images has been explored in several recent works. These approaches mainly rely on the photometric loss~\cite{back-to-basic}
\begin{equation}
\ell_{photometric}(I_s,I_t,V) = \rho(I_t, warp(I_s; V))
\end{equation}
to measure the difference between the target image and the inversely warped source image using the predicted flow. Here, $warp(\cdot;\cdot)$ denotes the inverse warping function and $\rho(x)={(x^2+\epsilon^2)}^\alpha$ is the Charbonnier penalty function~\cite{charbonnier}. 

Smoothness loss based on total-variation (TV)~\cite{ren2017unsupervised} is also employed to regularize the flow prediction:
\begin{equation}
\ell_{TV}(V) =  {\Vert \frac{\partial}{\partial x}V\Vert_1} + {\Vert \frac{\partial}{\partial y}V\Vert_1}.
\end{equation}

However, when conducting experiments, we found that plain training using the two losses on a single scale does not converge due to the large displacements on the pose guided dataset. Even after employing a multi-scale strategy, the trained flow often leads to a warped image with damaged  local structural details. We attribute this phenomenon to the poor ability of  $\ell_{photometric}$ and $\ell_{TV}$ to preserve the high-frequency structures of the warped image. To solve this issue for realistic pose-guided synthesis, we propose a structure-preserving objective function $\ell_{struct}$ that enforces structural similarity between the target image and the inversely warped source image:
%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\begin{aligned}
\label{eq:struct}
&\ell_{struct}(I_t, I_s, V)\\
=& G(\mathbf{f}_{vgg}^{(l)}(I_t))-G^l(\mathbf{f}_{vgg}^{(l)}(warp(I_s; V))) \Vert^2_2,
\end{aligned}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%
where $\mathbf{f}_{vgg}^{(l)}(\cdot)$ computes the $l$'th layer VGG~\cite{vgg} feature map of the given input image, and $\mathbf{G}^l(\cdot)$ denotes the Gram matrix~\cite{nerual_texture} to capture the second-order statistic of the given feature map. We select the VGG feature maps from layer \texttt{relu1\_2}, \texttt{relu2\_2},  \texttt{relu3\_2}, \texttt{relu4\_2} to compute the structural loss.

To enable convergence on the large displacement pose guided dataset, we use a multi-scale version of the three losses, which are then weighted summed to compute the final loss. Specifically, let $\{I^{(i)}_s\}$ and $\{I^{(i)}_t\}$  denote the re-scaled images of $I_s$ and $I_t$ at Gaussian pyramid level $i=[0,\dotsi ,5]$, the total loss is represented as: 
%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\begin{aligned}
\label{eq:stage1_loss}
\mathcal{L}_{Stage\RNum{1}}&(I_s,P_s,I_t,P_t,V) \\ 
= \sum_{i} s_i &(\ell_{photometric}(I^{(i)}_s,I^{(i)}_s,V^{(i)})  \\ 
& + \beta_i \ell_{struct}(I^{(i)}_s,I^{(i)}_s,V^{(i)}) + \gamma_i \ell_{TV}(V^{(i)})).
\end{aligned}
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%
To further improve convergence and regularize the learned flow, we employed a semi-supervised strategy~\cite{swapnet}. Specifically, let $A(\cdot)$ denote augmentation transformation based on cropping, affine transformation and flipping, the augmented source pose $A(P_s)$ and source image $A(I_s)$ are treated as target pose and target image, respectively. During training, $25\%$ percent of the training samples are selected from such synthetic target images and poses to help the model learn from the simple augmentation transformations first.

\subsection{Stage-\RNum{2}: Coarse-to-Fine Synthesis}
\begin{figure}[t]
	\centering
	\includegraphics[width=1.0\linewidth]{figures/Synthesis2.pdf}
	\caption{The network structure of SynthesisNet. Similar to GarmentNet, the SynthesisNet relies on multi-scale flow fields from Stage-\RNum{1} to spatially aligned the source domain encoding. The image output is then generated using the Unet decoder. The green, blue, yellow blocks indicate the source encoder, target encoder and Unet decoder, respectively.}
	\label{fig:synthesis_model1}
\end{figure}
Based on the learned flow estimator, we further propose GarmentNet and SynthesisNet to sequentially generate garment parsing and final image output following a coarse-to-fine pipeline. As shown in Figure \ref{fig:pipeline} and Figure \ref{fig:synthesis_model1}, GarmentNet and SynthesisNet share a unified network structure, which rely on the learned flow to align the source domain features following an U-Net decoder to fuse information from the source and target images. In addition, alpha blending is utilized at the end of the network to preseve the background.

Formally, GarmentNet (see Eq.~\ref{eq:clothnet}) takes the generated flow $\mathcal{V}=\{V^{(i)}|i=[0,\dotsi ,5]\}$, source garment $C_s$, source pose $P_s$, target pose $P_t$ and background garment parsing $C_{bg}$ \footnote{Since we are interested in transferring the garment style from the source rather than the face or hair shape of the target person, we take the  background garment parsing by the target face and hair region} as inputs and then output the target garment parsing $\hat{C}_t$:
%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\label{eq:clothnet}
	\hat{C}_t=GarmentNet(C_s, P_s, P_t, C_{bg},\mathcal{V}),
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%
whereas SynthesisNet (see Eq.~\ref{eq:synthesisnet}) takes $\mathcal{V}$, $I_s$, $C_s$, $P_s$, $\hat{C}_t$, $P_t$, and background image $I_{bg}$ \footnote{The background image refers to the inpainted non-body region as well as the hair and face of the target image.} as inputs, and then generates the final output $\hat{I}_t$.
%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\label{eq:synthesisnet}
\hat{I}_t=SynthesisNet(\hat{C}_t,I_s, P_s, P_t,I_{bg},\mathcal{V}).
\end{equation}
%%%%%%%%%%%v%%%%%%%%%%%
Since the two networks share the same network structure and have different inputs, we elaborate on the shared network structure in Sec.~\ref{subsection:method-stage2}.

\subsubsection{Network Structure}
\label{subsection:method-stage2}
As shown in Fig.~\ref{fig:flow_model} and \ref{fig:synthesis_model1}, our model relies on the source encoder and target encoder to respectively encode the features from source input and target input at multiple scales. We use 7 residue blocks at the end of source encoder for better feature extraction ability.

To perform alignment, the flow field is first generated at multiple scales using the trained flow estimator. Next, inverse warping is performed on the feature maps of the source encoder at all scales. 

After feature alignment, we employ a U-Net fusion decoder~\cite{crossnet} for feature aggregation. Unlike~\cite{crossnet} which directly concatenates two feature maps, we propose a multiplicative attention module to filter misaligned source features. Specifically, let $\mathbf{f}_s$ and $\mathbf{f}_t$ denote the warped source feature and target feature at the same location, the multiplicative attention filtering is defined as:
%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\label{eq:multiplicative_filter}
\mathbf{f}_s^\prime = \mathbf{f}_s \cdot \delta(\mathbf{f}_s^T \mathbf{W} \mathbf{f}_t),
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%
where $\delta$ represents the sigmoid function and $\mathbf{W}$ is learnable parameter. Such a filtering operation can be implemented on the 2-D feature map using $1\times1$ convolution, element-wise multiplication and summation. Please refer to the supplementary material for more details.

To avoid changing the given background content $bg$, our network simultaneously generates the foreground $fg$ content, along with a mask $M$ using the sigmoid activation function. The output is then computed as:
%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\label{eq:mask}
output = M \odot fg +  (1-M) \odot bg
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Training Objective and Details}
To train GarmentNet, we use the cross entropy loss between the ground truth garment $C_{gt}$ and prediction $\hat{C}_t$:
%%%%%%%%%%%%%%%%%%%%%%
\begin{equation}
\label{eq: cross_entropy_loss}
\mathcal{L}_{GarmentNet} = - \sum_{n} \mathbbm{1}(C_{gt}(i,j)=n) (\log \hat{C}_t(i,j))
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%
To train SynthesisNet, we use a combination of L1 loss, vgg feature loss, texture loss, and GAN loss. The training objective is represented as:
%%%%%%%%%%%%%%%%%%%%%%
\begin{align}
\label{eq: total_loss}
\mathcal{L}_{synthesisnet} &  = \lambda_{1} \ell_1  + \lambda_{2} \ell_{vgg} \nonumber \\
& + \lambda_{3} \ell_{struct} + \lambda_{4} \ell_{gan},
\end{align}
%%%%%%%%%%%%%%%%%%%%%%
where $\ell_1={\Vert \hat{I}_t - {I}_{gt} \Vert_1}$ computes the L1 differences, $\ell_{vgg}= \lambda_{1} \Vert f_{vgg}(\hat{I}_t) - f_{vgg}({I}_{gt}) \Vert_1$ computes the VGG feature difference on \texttt{relu4\_2} layer. $\ell_{struct}$ (Eq.~\ref{eq:struct}) computes texture-level similarities. Similar to ~\cite{cyclegan}, we replace the negative log-likelihood loss with least-square distance~\cite{lsgan} to compute the GAN loss $\ell_{gan}$. Specifically, the GAN los is defined as:
\begin{equation}
\ell_{gan} = {(D(I_t)-1)}^2 + {D(\hat{I}_t)}^2,
\end{equation}
where the discriminator ($D$) is implemented using a PatchGAN version~\cite{pix2pix} with spectrum normalization~\cite{sn}. $\lambda_1,\lambda_2,\lambda_3,\lambda_4$ are hyper-parameters, which control the relative importance of different loss term. We set $\lambda_1= 1.0, \lambda_2= 1e-4,\lambda_3=0.1,\lambda_4=0.5$ respectively in our experiments. 

% Finally, the training objective is represented as 
% \begin{equation}
% \arg \min_{G} \max_{D}\mathcal{L}_{synthesisnet}
% \end{equation}

\subsubsection{Background Content}
Since we are only interested in modifying the shape and appearance of the garment region rather than the face, hair or background, a masking scheme is employed as mentioned above. Here, we briefly describe the background generation procedure. The background for GarmentNet $C_{bg}$ contains only the garment parsing of hair and face of that person. As shown in Figure~\ref{fig:synthesis_model1}, to generate the background for SynthesisNet $I_{bg}$, we extract the background from the image and then perform inpainting~\cite{inpaint}. Afterward, the inpainted background as well as the hair and face content are treated as background and feed to the network.

%
%
%where $\ell_{photometric}$ re
%
%We employ a combination photometric loss and total variation loss at each scale,
%
%%\begin{equation}
%%warp(c^{(i)}, V^{(i)}).
%%\end{equation}
%
%
% under the challenging large body deformation, we designed a training 
%
%estimating the pose changes, therefore, the pose are used to compute
%
% Since the target image can vary in appearance, we use the more invariant target pose. In addition, we s 
%
%we use the $I_t$. To utilize person prior knowledge, we utilize Densepose~\cite{densepose} to generate source and target pose $P_s$
%
%
%
%The flow estimator we employed 
%
%To learning the texture preserving optical flow, we employ the FlowNetS~\cite{}. 
%
%
%Challenge: Large non-rigid, unsupervised, texture
%Solution: 
%pyramid auxiliary loss (gaussian kernel anti-aliasing)
%Gram loss
%TV loss
%semi supervised dataset

%\subsection{Two-stage synthesis network}
%Challenge: synthesis is challanging, therefor two-stage. 
%
%Key contribution:
%	loss: l1, vgg, gram, gan, auxiliary (chomobier loss)
%	auxiliary loss
%	mul attention
%	mask 

%\section{Approach}
%
%\begin{figure}
%	\centering
%	\includegraphics[width=1.0\textwidth]{figures/main.pdf}
%	\caption{(a): network structure of our proposed EWD-SRNet, (b): an image warping + synthesis pipeline for comparison }
%	\label{fig:model}
%\end{figure}
%
%Figure \ref{fig:model} summarizes the structure of our proposed EWD-SRNet (left) and compares it against an image warping + fusion pipeline (right) which resembles the network structure of~\cite{task_flow}~\cite{LFVideo}. Our key observations for EWD-SRNet are: 
%First, performing warping at only the finest scale slowdowns the convergence, as the flow-field vector is updated by only searching image (or feature) contents withing 1 block-matching distance from that vector. To enlarge the content searching space, we instead utilizes flow-fields from lower scales to higher scales to perform a sequential of warping operations. Second, performing warping and fusion on the raw-images domain is not optimal, because the raw LR and reference images do not specifically provide complementary and task oriented informations for fusion. Conversely, our model extract multi-scale feature maps from the LR image and reference image for feature-based warping and fusion.
%Finally, we proposed an decoder for feature fusion and synthesis using U-Net structure. Our decoder contains multiple skip connections between the flow-field estimator and the fusion module, which allows gradient to propagate easier from latter to former. Comparing to the image warping + fusion counterpart, our proposed model can be directly trained without pre-training the flow-field estimator.
%
%%Finally, the training dynamic of such model is further complicated by the fact that t update of the flow-estimator relies on the . training dynamic of such model is further complicated by the fact that the update of the flow-estimator relies on the. flow-field estimator is also hindered by the training . The training is complicated by the fact that the inputs to each layer are affected by the parameters of all preceding layers
%
%\subsection{Multi-scale Flow-field Estimator}
%As shown on the top of Figure \ref{fig:model}(a), given an bicubic upsampled LR image and its corresponding reference image, we adopt the widely used the FlowNetS~\cite{FlowNet} as our multi-scale flow-field estimator. To improve the FlowNetS, we made several modifications: firstly, the activation function of FlowNetS is change from ReLU to SELU~\cite{SELU} which considerably improves the model convergence; on the top of that, we additionally replace the final $\times 4$ bilinear upsampling layer of FlownetS with two deconvolution layer following skip connection layers for up-sampling the flow-field twice. The additional upsampling layers allows our modified model to output flow-field with much finner definition.
%
%\subsection{Reference Image Encoder}
%Given the reference image $I_R$, we designed a reference encoder to extract reference feature maps at 4 scales. Specifically, we convolves the raw reference images with 64 $5 \times 5$ filters with stride 1 to extract feature map at scale $0$. After that, we repeatedly convolves the feature map at scale $i-1$ (for $0 < i \le 3$) with with 64 $5 \times 5$ filters with stride 2 to extract feature map at scale $i$:
%
%%\begin{equation}
%\begin{eqnarray}
%	F^{(0)}_R &=& \delta(\boldsymbol{W}^{(0)}_R \ast I_R + \boldsymbol{b}^{(0)}_R), \\
%	F^{(i)}_R &=& \delta(\boldsymbol{W}^{(i)}_R \ast F^{(i-1)}_R + \boldsymbol{b}^{(i)}_R) {\Downarrow_2}, ~ i = {1,2,3}.
%\end{eqnarray}
%%\end{equation}
%
%\subsection{LR Image Encoder}
%Given the LR image, we utilize an single-image SR (SISR) approach~\cite{MDSR} to upsample the LR image to the same scale as the reference image. After that, an LR image encoder with the exact structure of the reference image encoder are employed to extract the LR image features maps. However, we allow the LR image encoder and the reference image encoder to learn different weights, which help the two sets of features to complement each other. 
%
%%\begin{equation}{l}
%\begin{eqnarray}
%SR_L &=& SISR(I_L), \\
%F^{(0)}_L &=& \delta(\boldsymbol{W}^{(0)}_L \ast SR_L + \boldsymbol{b}^{(0)}_L), \\
%F^{(i)}_L &=& \delta(\boldsymbol{W}^{(i)}_L \ast F^{(i-1)}_L + \boldsymbol{b}^{(i)}_L) {\Downarrow_2}, ~ i = {1,2,3}.
%\end{eqnarray}
%%\end{equation}
%
%Utilizing independent SISR approaches (such as~\cite{MDSR} ) to encode LR image has two advantages: First, the SISR approaches that are validated on large-scale external datasets helps the LR image encoder to generalize better on unseen scenes; second, new state-of-the-art SISR approaches can be easily integrated into our system to improve performance without changing our network structures.
%
%\subsection{Flow Estimator}
%We applied a modified FlownetS~\cite{FlowNet} as our flow estimator. Specifically, to increase the flow precision, we replace the final $\times4$ bilinear upscaling layer of FlownetS with two deconvolution layer using skip connection for $\times2$ upscaling. The modified flow estimator is used to generate the multi-scale flow.
%
%\begin{eqnarray}
%\{V^{(3)}, V^{(2)}, V^{(1)}, V^{(0)}\} = {Flow}(I_L, I_R)
%\end{eqnarray}
%
%
%\subsection{Decoder using Fusion}
%After extracting multi-scale image features and the corresponding flow-fields at different scales, we warp the reference feature using backward warping at every scales. 
%
%\begin{eqnarray}
%	F^{(i)}_{Rw} = warp(F^{(i)}_R, V^{(i))}), ~ i = {0,1,2,3}.
%\end{eqnarray}
%
%
%After that, a U-Net like decoder is proposed to perform fusion and SR synthesis. Specifically, the warped features and the LR image features at scale $i$ (for $0 < i \le 3$), as well as the decoder feature from scale $i-1$ are concatenated following a deconvolution layer with 64 $4 \times 4$ filters and stride 2 to generate decoder features at scale $i$. 
%
%\begin{eqnarray}
%F^{(3)}_{d} &=& \delta(\boldsymbol{W}^{(3)}_{d} \star (F^{(3)}_L, F^{(3)}_{Rw}) + \boldsymbol{b}^{(3)}_{d}), \\
%F^{(i)}_{d} &=& \delta(\boldsymbol{W}^{(i)}_{d} \star (F^{(i+1)}_L, F^{(i+1)}_{Rw}, F^{(i+1)}_{d}) + \boldsymbol{b}^{(i)}_d), ~ i = {2,1,0}.
%\end{eqnarray}
%
%After generating the decoder feature at scale $0$, 3 additional convolution layers with filter sizes $5 \times 5$ and filter number $\{64,64,3\}$ are added to synthesis the SR output. 
%
%\begin{eqnarray}
%F^{}_{1} &=& \delta(\boldsymbol{W}^{(0)}_p \ast F^{(i)}_{d} + \boldsymbol{b}^{(0)}_p), \\
%F^{}_{2} &=& \delta(\boldsymbol{W}^{(0)}_p \ast F^{}_{1} + \boldsymbol{b}^{(0)}_p),	\\
%I_p &=& \delta(\boldsymbol{W}^{(0)}_p \ast F^{}_{2} + \boldsymbol{b}^{(0)}_p).
%\end{eqnarray}
%
%\subsection{Loss Function}
%Our network can be directly trained to synthesis the SR output. Given the reference image $I_{R}$, the LR image $I_{L}$, the network prediction $I_{p}$ and the ground truth image $I_{H}$, the loss function can be written as:
%
%\begin{eqnarray}
%	\mathcal{L} = \frac{1}{N} \sum_{i=1}^{N} \sum_{s} \rho (I_{H}^{(i)}(s) - I_{p}^{(i)}(s) ),
%\end{eqnarray}
%
%where $\rho(x)=\sqrt{x^2+0.001^2}$ is the Charbonnier penalty function~\cite{Charbonnier}, N is the number of samples, $i$ and $s$ iterate over training samples and spatial locations respectively.
%
%

